Recurrence and transience for the frog model on trees

The frog model is a growing system of random walks where a particle is added whenever a new site is visited. A longstanding open question is how often the root is visited on the infinite $d$-ary tree. We prove the model undergoes a phase transition, finding it recurrent for $d=2$ and transient for $d\geq 5$. Simulations suggest strong recurrence for $d=2$, weak recurrence for $d=3$, and transience for $d\geq 4$. Additionally, we prove a 0-1 law for all $d$-ary trees, and we exhibit a graph on which a 0-1 law does not hold. To prove recurrence when $d=2$, we construct a recursive distributional equation for the number of visits to the root in a smaller process and show the unique solution must be infinity a.s. The proof of transience when $d=5$ relies on computer calculations for the transition probabilities of a large Markov chain. We also include the proof for $d \geq 6$, which uses similar techniques but does not require computer assistance.

==> intro25__Matthew_Junge_s_conflicted_copy_2016-04-17_.tex <==
%!TEX root = frog_paper.tex

The frog model is a system of interacting random walks on a given rooted graph.
Initially, the graph contains one particle at the root and
some configuration of sleeping particles on its vertices;
unless otherwise stated, we will assume an initial condition of one sleeping particle per vertex.
The particle at the root starts out awake and performs a simple nearest-neighbor random walk in discrete time.
Whenever a vertex with sleeping particles is first visited, all the particles at the site wake up
and begin their own independent random walks, waking particles as they visit them.
A formal definition of the frog model is in \cite{shape}, and a nice survey of variations is in \cite{frogs}.
Traditionally, particles are referred to as frogs, a practice we will continue here.

One of the most basic questions about the frog model on an infinite graph is whether it is 
recurrent or transient. Telcs and Wormald determined that the frog model was recurrent on $\ZZ^d$ for
any $d$, the first published result on the frog model \cite{telcs1999}. 
On an infinite $d$-ary tree, this question is more difficult.
It was first posed in \cite{phasetree}. It was asked again in \cite{frogs} and
in \cite{recurrence}, which pointed out that the answer was unknown even on a binary tree.

Our main result in this paper is that the frog model is recurrent on the binary tree
but transient on the $d$-ary tree for $d\geq 5$, demonstrating a phase transition not found on $\ZZ^d$.
A branching random walk martingale argument proves transience when $d \geq 6$. Pushing this result
down to $d=5$ is more complicated and requires computer assistance.
Our proof of recurrence on the binary tree uses a bootstrapping argument in which we iteratively
assume that the number of visits to the root is stochastically large and then prove it even
larger; the argument seems novel to us.

\subsection*{Background on the frog model}

 It is common to use the frog model as a model for the spread of rumors or infections, thinking of awakened frogs as informed or infected agents. See \cite{daley} for an overview and \cite{epidemic} for more tailored discussion. 
 Another perspective on the frog model is as a conservative lattice gas model with the reaction $A + B \to 2 A$. Here $A$ represents an an active particle and $B$ an inert particle. Active particles disperse throughout the graph, igniting any inert particles they contact. 
Several papers taking this perspective study a process identical to the frog model except that particles
move in continuous rather than discrete time \cite{sid04,CQR,BR}. 
This process and its variants have also seen much study by physicists; see the references in \cite{CQR}
and \cite{BR}. Our results in this paper depend
only on the paths of the frogs and not on the timing of their jumps,
and so they apply equally well to this continuous-time process.
 
 
In the larger mathematical context, the frog model is part of a family of self-interacting random walks which have proven quite difficult to analyze. (\cite{pemantlesurvey} provides a nice survey of this family.)
In recent years progress on a few self-interacting random walks has generated considerable interest.  
One of these close relatives is activated random walk, which is touched on
in \cite{KS} and studied in depth in \cite{DRS,RS,ST}.  %,Shellef,AmirGG,CRS}.
Activated random walk can be described as a frog model where frogs fall back asleep
at some given rate. 
Another related process is excited random walk \cite{excited}.
This walk has a bias the first time it visits a site but is unbiased each subsequent time that it returns.
The frog model can be thought of as an ``excited" branching process, which branches at a site $v$ only the first time the process visits $v$.
 




Initial interest in the frog model was on the graph $\ZZ^d$. For any $d$, it was shown that the process
is recurrent \cite{telcs1999} and that the set of visited vertices grows linearly and when rescaled
converges to a limiting shape \cite{shape}. A similar shape theorem was proven independently in \cite{sid04} 
for the process with continuous-time particles.
Both shape theorems rely on the subadditive ergodic theorem. A technical difficulty that arises is proving the expected time to wake a given frog is finite. Thus, measuring recurrence on a given graph is the first step in understanding the long time behavior of the model. Transience and recurrence continue to attract attention. Also on $\mathbb Z^d$, \cite{random_frog} establishes the frog model %on $\ZZ^d$ 
undergoes a phase transition from transience to recurrence depending on how the number of frogs per site decays proportional to distance to the origin. 
%as the initial density of sleeping frogs is increased
%Transience and recurrence are also studied for
Phase transitions are also established when frogs walk with   a bias in one direction. This is studied on $\mathbb{Z}$ in \cite{recurrence} and on
$\mathbb{Z}^d$ in \cite{dobler2014} and \cite{01frog}.

%, 
%When the walks have a bias in one direction: \cite{recurrence} finds that on $\mathbb Z$,
%  the model is recurrent if and only if the number of sleeping frogs per site has infinite logarithmic moment.
%  A sufficient condition for recurrence in this setting on $\mathbb{Z}^d$ was given in \cite{dobler2014} and 
%  improved on in \cite{01frog}.



% Later this question was studied on the integers with drift \cite{recurrence}. A more general analysis in this setting recently appeared in \cite{dobler2014} and \cite{integers_drift2}. 


Our main interest in this paper is in recurrence and transience on $\mathbb T_d$, the infinite rooted $d$-ary tree. We denote the root by $\emptyset$. 
We also study aspects of the process on $\homtree_d$, the infinite
homogeneous degree $(d+1)$-tree. 
 




%Intuitively, the frog model ought to outpace a single random walk. 
%Most of the results about the frog model have been when the underlying graph is $\mathbb Z^d$. Here the frog model is recurrent for all $d$ and the set of activated vertices (properly scaled) converges to a convex region (see \cite{telcs1999} and \cite{shape}). 



%, in which every vertex has degree~$d+1$. 
%Our choice to study the model on $\TT_d$ may at times appear cumbersome, but it greatly facilitates our discussion of finite trees. Also, since the the techniques we apply to $\TT_d$ export nicely to $\homtree_d$ we are working in slightly more generality.


Some attention has already been given to a relative of our model on $\homtree_d$
in which awake frogs die after independently taking a geometrically distributed number of jumps.
In \cite{phasetree} and \cite{po2}, the authors prove a phase transition for survival. Depending on the parameter, there will either be frogs alive at all times with positive probability or the process will die out almost surely. We study the model in which frogs jump perpetually---a fundamentally different problem, since it switches the emphasis from the local to the global behavior of the model. 






\subsection*{Statement and discussion of results}
For a given rooted graph we call a realization of the model recurrent if the root is visited infinitely many times and transient if it is visited finitely often. 
%If either of these happens with probability one then we say the frog model is recurrent or transient. 
Our main theorem covers the $d$-ary tree for all but two degrees:

\begin{thm}\thlabel{thm:2tree} \thlabel{thm:5tree} \ \

\begin{enumerate}[(i)]
    \item The frog model on $\TT_2$ is almost surely recurrent.\label{d2}
    \item  The frog model on $\TT_d$ for $d \geq 5$ is almost surely transient.\label{d5}
\end{enumerate}

\end{thm}

We also make a conjecture on these two unsolved degrees
based on fairly convincing evidence from simulations, presented
in Section~\ref{sec:conjectures}. %we cannot analyze in Theorem \ref{thm:2tree}.
\begin{conjecture}\thlabel{conj:phase_transition}
  The frog model on $\TT_d$ is recurrent a.s.\ for $d=3$ and transient 
  a.s.\ for $d= 4$.
\end{conjecture}

The simulations suggest the possibility of a three-phase transition as $d$ increases. 
We call the model strongly recurrent if the probability the root is occupied is bounded away from zero
for all time.
We call it weakly recurrent if it is recurrent with positive probability, but the probability
that the root is occupied decays to zero.



\begin{question} \label{q:strong_weak}
Is the frog model strongly recurrent on $\TT_2$ but weakly recurrent on $\TT_3$?
\end{question}

Such a transition would give information about the time to wake all children of the root. For instance, strong recurrence on $\TT_2$ would imply that this time has finite expectation and an exponential tail. Should $\TT_3$ exhibit a weak recurrence phase, then a tantalizing problem would be to estimate the decay of the occupation time at the root.  


The recurrence of the frog model on the binary tree established in \thref{thm:2tree}~(\ref{d2}) is the flagship 
result of this article. 
%First we give a general idea of the proof and discuss its significance. A slightly more technical outline follows. 
%The idea of our proof is as follows.
The proof goes by coupling the frog model with a process in which the root is visited less often. Let $V$ be the number of visits to the root in this restricted model. 
The payoff is \eqref{eqn:keyform}, a recursive distributional equation (RDE, see \cite{AB}) relating $V$ and two independent copies of itself. We find that $V\sim \delta_{\infty}$ is the unique solution. Thus, the original model is recurrent. 

The proof that $V\sim\delta_{\infty}$ is the unique solution of the RDE
uses a seemingly novel bootstrapping argument. 
We assume that $V$ dominates a Poisson  and show that in fact, $V$ dominates a Poisson with slightly
larger mean. It follows by repeating this argument that $V$ dominates any Poisson. 
One obstacle to making this work is that using the typical definition of stochastic dominance,
we cannot establish a base case for the argument.
To get around this, we instead use a weaker stochastic ordering defined in terms of generating functions,
under which the argument holds even when starting with the trivial base case of $V$ dominating 
the distribution $\Poi(0)$.
The situation is different for the frog model with initial conditions of $\Poi(\mu)$ frogs per site.
In this setting, we use the usual notion of stochastic dominance and a related
bootstrapping argument to prove a phase
transation from transience to recurrence on any $d$-ary tree as $\mu$ increases \cite{frog2}.



 
We believe that these ideas are more widely applicable.
Aldous and Bandyopadhyay study RDEs in general in \cite{AB}. 
Another example of analyzing an RDE
through an induced relation of generating functions can be found in \cite{Liu}.
The RDE~\eqref{eqn:keyform} in this paper is specific to our setting and much more complicated than the RDEs analyzed
in either of these sources. Still, we think that our argument can be applied to other RDEs,
including ones derived from similar interacting particle systems
like activated random walk and the frog model with death.
   
   
 %An important difference is that these related models exhibit more serious time dependence.
% Compare to the frog model which depends exclusively on the range of walkers. 
%Another contribution of our paper is the proof of a unique fixed point.
% $\delta_{\{\infty\}}$.
%The use of bootstrapping and a more exotic stochastic order appear to be novel and may help analyze general processes. 


For the transience part of \thref{thm:2tree}, the idea is to dominate the frog model by a branching process. At the beginning of Section~\ref{sec:transience}, we show in a few lines that a doubling branching random walk is transient on the $15$-ary tree. A simple refinement in \thref{prop:6tree} improves this to $d \geq 6$. The case $d=5$ uses a branching random walk with 27 particle types. This is significantly more complicated,
and computing the transition probabilities requires computer assistance. Conceptually our approach could extend to a computer-assisted proof for transience when $d=4$, but the demands of this theoretical program seem well beyond current processing power. 

% On the binary tree ($d=2$), we couple the frog model with a process that visits the root less often. The probability generating function for the number of visits to the root by this process satisfies a recursive relation. 
%We then use an analytic argument to prove
%the generating function is identically zero, or equivalently, the probability of infinitely many visits is 1.
%The approach seems novel; we discuss it more in \thref{rmk:RDE}.

%For $d \geq 5$, we compare the frog process to a branching random walk that dominates the frog process but is still transient. The proof for 
%$d\geq 6$ is fairly short, while for $d=5$ it needs computer assistance. 

%In \thref{prop:6tree,prop:5.5tree}, we give slightly weaker results
%using
%the same ideas
%but no difficult calculations.

We present two other results besides Theorem~\ref{thm:2tree}.
The first is a 0-1 law for transience and recurrence of the frog model on a $d$-ary tree that
applies under more general initial conditions than one frog per site.
For a given distribution $\nu$ on the nonnegative integers, we consider the frog model on a $d$-ary
tree with the number of sleeping frogs on each vertex other than the root drawn independently
from $\nu$. The root initially contains one frog, which begins its life awake. Recall that when a site is
visited for the first time, all sleeping frogs at that site are awoken. We refer to this as
the frog model with i.i.d.-$\nu$ initial conditions. When $\nu=\delta_1$, this is the usual one-per-site
frog model. This theorem complements the 0-1 law for recurrence proven in \cite{recurrence} 
in a frog model on $\Z$ with drift. It also plays an important role in \cite{frog2}, where we use it to show
that the probability of recurrence for the frog model on a $d$-ary tree with i.i.d.-$\Poi(\mu)$
initial conditions jumps abruptly from 0 to 1 as $\mu$ increases. More recently, \cite{01frog} proved a 0-1 law for the frog model that applies in a wide range of circumstances. For instance, it establishes that recurrence holds either with probability~$0$ or $1$ for the frog model on any transitive graph. This would apply immediately here if we worked on the $(d+1)$-regular tree rather than the rooted $d$-ary tree. 


 

\begin{thm}\thlabel{thm:01law}
 The frog model on $\TT_d$ for any $d$ and any i.i.d.\ initial conditions is
 recurrent with probability 0 or 1.
\end{thm}


Our final related result is that in contrast to the 0-1 law on $\TT_d$, there is a 
graph on which the frog model is recurrent with probability strictly between $0$ and $1$. 






\begin{thm} \thlabel{thm:counterexample}
Let $G$ be the graph formed by merging the root of $\TT_6$ and the origin of $\mathbb Z$ into one vertex. The frog model on $G$ has probability $0<p<1$ of being recurrent. 
\end{thm}



We remark that \cite{random_frog} exhibits a frog model without a 0-1 law on $\ZZ^d$. In their example the
initial distribution of frogs decays in the distance from the origin. 
 %To our knowledge \thref{thm:5tree}~(\ref{d5}) provides the first example of a graph on which the one-frog-per-site model is transient, which is key to our construction in \thref{thm:counterexample}.


A few of our proofs would be simplified by changing the setting from $d$-ary to homogeneous trees. However, 
we are interested in applying these results to 
finite trees, and the infinite $d$-ary tree is more natural to work with from that perspective. In any event, the techniques 
underlying our theorems can all be cleanly modified to prove similar 
statements about the homogeneous tree.
%\begin{question} \label{q:gw}
%Is the frog model a.s.~recurrent on a Galton-Watson tree in which parents can produce two offspring?
%\end{question}








